Experimental investigation of the effect of ionization on the 51V(p,n)51Cr reaction

The investigation of the effects of average atomic ionization on nuclear reactions is of prime importance for nuclear astrophysics. No direct experimental measurement using a plasma target has been done yet. In this regard, we measured for the first time the neutron production of a (p,n) reaction in different states of ionization. The studied nuclear reaction was 51V(p,n)51Cr. We measured a significantly lower neutron production than expected when the target was ionized, even when taking into account existing electron screening theory or the effect of the stopping power in the target on the injected proton beam. This experiment is a first step in the process to characterize the influence of ionization at astrophysically relevant energies.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


